VECSEL systems for quantum information processing with trapped beryllium ions

Two vertical-external-cavity surface-emitting laser (VECSEL) systems producing ultraviolet (UV) radiation at 235 nm and 313 nm are demonstrated. The systems are suitable for quantum information processing applications with trapped beryllium ions. Each system consists of a compact, single-frequency, continuous-wave VECSEL producing high-power near-infrared light, tunable over tens of nanometers. One system generates 2.4 W at 940 nm, using a gain mirror based on GaInAs/GaAs quantum wells, which is converted to 54 mW of 235 nm light for photoionization of neutral beryllium atoms. The other system uses a novel gain mirror based on GaInNAs/GaAs quantum-wells, enabling wavelength extension with manageable strain in the GaAs lattice. This system generates 1.6 W at 1252 nm, which is converted to 41 mW of 313 nm light that is used to laser cool trapped $^{9}$Be$^{+}$ ions and to implement quantum state preparation and detection. The 313 nm system is also suitable for implementing high-fidelity quantum gates, and more broadly, our results extend the capabilities of VECSEL systems for applications in atomic, molecular, and optical physics.

==> outline.tex <==
Comparing the performances of lasers in the refs for VECSEL paper

Solid-state lasers:

	1. A.C.Wilson et al.  (2011)
A 750-mW, continuous-wave, solid-state laser source at 313 nm
for cooling and manipulating trapped 9Be+ ions:
750 mW@313nm, 
5 W at 1550 and 1051 nm -> 2W@626nm (a conversion efficiency of 24%), 495-GHz range for UV, narrow-linewidth,

	1. Hsiang-Yu Lo et al.  (2013)
All-solid-state continuous-wave laser systems for ionization,
cooling and quantum state manipulation of beryllium ions.:
400mW at 470 nm and 28mW at 235 nm.
7.2 W at 626 nm and 1.9 W at 313 nm are obtained using two pump beams at 1051 and 1551 nm.

Diode laser:
	1. Toptica laser (2013) - TA-SHG pro (High-power, tunable, frequency-doubled diode laser): 800mW at 626 nm, 10nm coarse tuning
	Toptica TA-FHG pro(High-power, tunable, frequency-quadrupled diode laser): 300mw@313nm 2nm coarse tuning
	2. H. Ball et al. (2013)
	A high-power 626 nm diode laser system for Beryllium ion trapping (2013):
	130mW near 626 nm, 3-5mw @ 313nm, required low temperature
	3. F. M. J. Cozijn et al (2013)
	Laser cooling of beryllium ions using a frequency-doubled
	626 nm diode laser:
	32mw @626 and 10mw -> 313.13 nm of 35 μW
	4. Ryan A. Carollo et al. (2017)
	Third-harmonic-generation of a diode laser for quantum control of beryllium ions:
	36mW at 313nm, complicated third-harmonic generation.
	
	



First VECSEL demonstration for this wavelength.
VECSEL advantages:
	i. Fairly simple system
	ii.  low cost and complexity (how much?)
	iii.  power-scalable.
	iv.  ??

Laser config:
I-cavity + doubling stages + frequency locking
Detailed configuration (Shaun)
Gain chip (J.P.)

Result:
Power curve (multi-mode, single mode at 1231nm, 1252nm, 626nm).
Line width.
Use VECSEL for laser cooling and detection. Res spectrum and repumping.

Preferred journal:
LPR- Laser and Photonics Reviews
Original Papers: The journal also welcomes original papers of high quality and originality. A length of about 35,000 characters (with spaces) or 5,000 words incl. references, excl. figures is recommended. This corresponds to 6–12 print pages. Lengthy derivations are requested to be submitted as additional material which will be published online as Supporting Information.


From J.P:
Based on the instructions, the letter length is 3-4 pages and original 6-12 pages. I skimmed through some papers and the 1252nm-313nm work should blend in quite nicely.
Attached a few recent articles from the journal as an example:
-          Zhang et.al. (letter) and Kumari et.al (original) describe lasers at new wavelengths and power records and with new characteristics but with preliminary results
-          I added Hong et.al (original), because I think we could also add quite nice schematic diagram of the system
 
You mentioned about writing a sort of recipe type of paper. How detailed you are thinking? We would of course explain:
-          The gain chip; quantum wells, processing, etc, on a general in few paragraphs – but it is sort of impossible to explain in detail how to manufacture chips
-          The VECSEL principles; cavity, wavelength filtering, cooling, closed casing – what else?
-          Wavelength locking
-          Doubling to visible
-          Doubling to UV and UV beam delivery (Panyu: cite Wilson et al. 2011 )
 
Depending on the “A-data”, we could highlight of course the power and the practicality of the setup – if you indeed find the setup practical.
 
As a closing remark, we could state that we have demonstrated Mg before, now Be(Panyu: cite Ting rei's mixed species gate paper),  and mention future possibilities with other ions and neutral atoms.


Paper structure (including 940 VECSEL):
Requirement of LPR: 
	1.  6-12 pages, 5000 words.
	2. Abstract: should be no longer than 200 words. Please use impersonal or passive style instead of the active “we” form.
	Please also submit an abstract text for the Table of Contents. It should be a maximum of 70 words, and should be written in impersonal or passive style. Up-load as "Production Data".
	3. Figures should preferably be submitted in full color, but should also be easily readable on a black/white printout. They need to be uploaded as separate files in a graphic format such as TIFF, EPS or JPG with a resolution of 300 dpi or higher (see ‘Artwork’). For graphic files choose the designation "Production Da-ta" on the File Upload screen in Editorial Manager.
	4. LaTeX users: Revisions must still be uploaded as a single PDF generated from the revised source files. Please use the File Designation "*Revised Manu-script" from the dropdown box. In addition please upload your TeX source files including bbl and figure files. For all source files the File Designation "Pro-duction Data" must be used. Previous versions of uploaded documents must be deleted. If the manu-script is accepted for publication the uploaded files will be used to typeset the article within a totally digi-tal workflow.
	5. Ref: please give the names of all authors

	



Title: High-power, continuous-wave VECSEL systems  for trapped beryllium ions

Abstract: 

Intro:  
	Paragragh1: 
	Trapped ions for QIP is important, and requires laser. 
	Among alkali ions, Be is the best but requires 313nm and 235 nm which is hard.
	Introduce Be structure and show a figure here to address the use of VECSEL in this work. Or move it in the start of "demonstration on Be ions"
	
	P2:
	Before, people use laser A, laser B, laser C but with different disadvantages.
	A good option is VECSEL demonstrated by Shaun.
	
	P3:
	We did… 

System description: 
	Part 1: VECSEL 1252 and performance results.
	
	Part 2: VECSEL 940 and performance results.
	
	describe each VECSEL system and characterize the performance such as power curve and line width. 

Demonstration on Be ions: 
	Part 1: using 1252 VECSEL to do
	laser cooling, res spectroscopy, repump;
	Part 2: using 940 VECSEL to do 
	Ionizing and count ion with channeltron.

Conclusion: 
	Address we have done
	Drawbacks and solutions : power is not as high as fiber laser but still scalable, may get higher power with higher input power.  large detuning (compare with 900GHz in high-fidelity paper) for reducing spontaneous emission with higher power.
	Further to do: potential to do mixed species experiment. Application on other species experiment. 

















